Software Verification for Weak Memory via Program Transformation

Despite multiprocessors implementing weak memory models, verification methods often assume Sequential Consistency (SC), thus may miss bugs due to weak memory. We propose a sound transformation of the program to verify, enabling SC tools to perform verification w.r.t. weak memory. We present experiments for a broad variety of models (from x86/TSO to Power/ARM) and a vast range of verification tools, quantify the additional cost of the transformation and highlight the cases when we can drastically reduce it. Our benchmarks include work-queue management code from PostgreSQL.

==> cycles.tex <==
\section{Looking for weak memory specific bugs \label{cycles}}

We now explain how we use \mythm\ref{thm:equiv} to develop verification
techniques for programs running on weak memory. Our first step is to compute an
over-approximation of the delayed pairs of all possible executions of the
program. To do so, we compute the \emph{control flow graph} (\cfg) of the
program, then its possible critical cycles. Then, the possible delayed events
are the ones that belong to a critical cycle of the \cfg.

Note that \mythm\ref{thm:equiv} forces a delayed write $w$ to stay
in the buffer as long as:
\begin{description}
\item[\dwpo] the events delayed before $w$ in program order and forming a safe pair with $w$ have not been flushed by \mfg; and
\item[\dwws] the writes to the same location (whether from the same thread or
not) and buffered before $w$ have not been flushed by \mfg;
\item[\dwrffr] if there is no such write, as long as the reads reading from
either the memory or from $w$ are delayed by \mfng.  \end{description}

Similarly, a delayed read $r$ stays in the queue as long as:
\begin{description}
\item[\dr] the events delayed before $r$ in program order and forming a safe
pair with $r$ have not been flushed by \mfg; and
%\item the reads from the same location and enqueued before $r$ have not been flushed (by \mfmfg~ and $\uniproc$).
\end{description}
\fixme{jade: check for both write and read if that's exhaustive}

Thus in the general case, there might be too many writes and reads being
delayed for us to verify a piece of code efficiently, if at all.
\fixme{jade@Michael: if we speak about decidability/complexity stuff, maybe
that's the place to do it?}

To overcome the difficulties sketched above, we look at specific parts of the
program, where the number and size of the delay devices can be bounded.

We recall the definition of critical cycles. Given an architecture $A$ and
event structure $E$, a cycle $\sigma$ amongst the events of $E$ is
\emph{critical} on $A$, when there is at least one delay pair $(e_1,e_2) \in
\sigma$ (as defined in \mysec\ref{instrumentation}) and $\sigma$ satisfies the
two following properties. \ccpo Per processor, there are at most two
memory accesses $(e_1,e_2)$ on this processor and $\loc(e_1) \neq \loc(e_2)$.
\ccloc For a given memory location $x$, there are at most three
accesses relative to $x$, these accesses are from distinct processors, and at
least one of them is a write (\ie $(w,w)$, $(w,r)$, $(r,w)$ or $(r,w,r)$). For
example in \myfig\ref{fig:sb}, the execution of \ltest{sb} has a critical cycle
on TSO.  In \myfig\ref{fig:iriw}, the execution of \ltest{iriw} has a critical
cycle on Power. 

Let us now consider a given critical cycle, assuming that all preceding events
(in program order) were memory events or have been flushed before we enter the
cycle. 

In this case, in the worst case, all delayed reads have to wait before the
preceding access in program order is flushed, following the clause \dr.

For delayed writes, the definition of critical cycle assures us that along the
cycle, for a given variable $x$, we have the following possible configurations.
In the worst case, all accesses are delayed and are the second access in
program order on their respective processor, with the preceding access being
also delayed:
\begin{description}
\item[$(w,w)$] we need two slots in the buffer for $x$, and we need to keep
these writes in the buffer for at most three steps of the machine (one step for
each access preceding a write in program order, and one step for the first
write flushed);
\item[$(r,w)$ or $(w,r)$] we need one slot in the buffer for $x$ and one in the
queue for $x$, and we need to keep these accesses delayed for at most three
steps of the machine (one step for each preceding access in program order, and
one step for the first access flushed);
\item[$(r,w,r)$] we need one slot in the buffer for $x$ and two in the
queue for $x$, and we need to keep these accesses delayed for at most five
steps of the machine (one step for each preceding access in program order, and
two steps for the first two accesses flushed)
\end{description}
\fixme{jade: NB the age bound (the number of steps) is really rough}

Now, when all the critical cycles of a program are disjoint, we can keep the
buffers and queues bounded by two, and flush them as soon as we exit the
critical cycle.
\fixme{jade@Michael: this corresponds to the picture with blobs that we drew in
the office; we replace a cycle by its SC-instrumented equivalent}


==> figures.tex <==
% vi: filetype=tex spell spelllang=en_gb:
\begin{figure}
  \centering
  \scalebox{1.0}{
  \begin{tikzpicture}[>=stealth,thin,inner sep=0pt,text centered,shape=rectangle]
  \useasboundingbox (0cm,0.5cm) rectangle (2cm,-2cm);
  
    \begin{scope}[minimum height=0.5cm,minimum width=0.5cm,text width=1.0cm]
      \node (a)  at (0, 0)  {\lb aWx{1}};
      \node (b)  at (0, -2)  {\lb bRy{0}};
      \node (c)  at (2, 0)  {\lb cWy{1}};
      \node (d)  at (2, -2)  {\lb dRx{0}};
    \end{scope}
		
    \path[->] (a) edge [out=225,in=135] node [left=0.1cm] {po} (b);
    \path[->] (b) edge [out=15,in=195] node [pos=0.8, below right=0.07cm] {fr} (c);
    \path[->] (c) edge [out=-45,in=45] node [left=0.1cm] {po} (d);
    \path[->] (d) edge [out=165,in=-15] node [pos=0.8, below left=0.07cm] {fr} (a);
  \end{tikzpicture}}
  \caption{SB}
  \label{fig:some}
\end{figure}

\begin{figure}
  \centering
  \scalebox{1.0}{
  \begin{tikzpicture}[>=stealth,thin,inner sep=0pt,text centered,shape=rectangle]
  \useasboundingbox (0cm,0.5cm) rectangle (2cm,-2.7cm);
  
    \begin{scope}[minimum height=0.5cm,minimum width=0.5cm,text width=0.8cm]
      \node (da)  at (0, 0)  {$\Del(a)$};
      \node (fa)  at (0, -0.5)  {$\Flush(a)$};
      \node (db)  at (0, -2)  {$\Del(b)$};
      \node (fb)  at (0, -2.5)  {$\Flush(b)$};
      \node (dc)  at (2, 0)  {$\Del(c)$};
      \node (fc)  at (2, -0.5)  {$\Flush(c)$};
      \node (dd)  at (2, -2)  {$\Del(d)$};
      \node (fd)  at (2, -2.5)  {$\Flush(d)$};
    \end{scope}
		
    \path[->] (da) edge [out=225,in=135] node [left=0.1cm] {po} (db);
    \path[->] (fb) edge [out=15,in=195] node [pos=0.8, below right=0.07cm] {se} (fc);
    \path[->] (dc) edge [out=-45,in=45] node [left=0.1cm] {po} (dd);
    \path[->] (fd) edge [out=165,in=-15] node [pos=0.8, below left=0.07cm] {se} (fa);
  \end{tikzpicture}}
  \caption{SB}
  \label{fig:some}
\end{figure}

\begin{figure}
  \centering
  \scalebox{1.0}{
  \begin{tikzpicture}[>=stealth,thin,inner sep=0pt,text centered,shape=rectangle]
  \useasboundingbox (0cm,1cm) rectangle (6cm,-2.5cm);
  
    \begin{scope}[minimum height=0.5cm,minimum width=0.5cm,text width=1.0cm]
      \node (a)  at (0, 0)  {\lb aRx{1}};
      \node (b)  at (0, -2)  {\lb bRy{0}};
      \node (c)  at (2, 0)  {\lb cRy{1}};
      \node (d)  at (2, -2)  {\lb dRx{0}};
      \node (e)  at (4, 0)  {\lb eWx{1}};
      \node (f)  at (6, 0)  {\lb fWy{1}};
    \end{scope}
		
    \path[->] (a) edge [out=225,in=135,dashed] node [left=0.1cm] {po} (b);
    \path[->] (c) edge [out=225,in=135,dashed] node [left=0.1cm] {po} (d);
    \path[->] (e) edge [out=150,in=30] node [above=0.1cm] {rf} (a);
    \path[->] (b) edge [out=-30,in=225,looseness=1.0] node [below right=0.07cm] {fr} (f);
    \path[->] (f) edge [out=150,in=30] node [above=0.1cm] {rf} (c);
    \path[->] (d) edge [out=30,in=-120] node [above left=0.07cm] {fr} (e);
  \end{tikzpicture}}
  \caption{IRIW+dps}
  \label{fig:some}
\end{figure}

\begin{figure}
  \centering
  \scalebox{1.0}{
  \begin{tikzpicture}[>=stealth,thin,inner sep=0pt,text centered,shape=rectangle]
  \useasboundingbox (0cm,1cm) rectangle (6cm,-3cm);
  
    \begin{scope}[minimum height=0.5cm,minimum width=0.5cm,text width=0.8cm]
      \node (da)  at (0, 0)  {$\Del(a)$};
      \node (fa)  at (0, -0.5)  {$\Flush(a)$};
      \node (db)  at (0, -2)  {$\Del(b)$};
      \node (fb)  at (0, -2.5)  {$\Flush(b)$};
      \node (dc)  at (2, 0)  {$\Del(c)$};
      \node (fc)  at (2, -0.5)  {$\Flush(c)$};
      \node (dd)  at (2, -2)  {$\Del(d)$};
      \node (fd)  at (2, -2.5)  {$\Flush(d)$};
      \node (de)  at (4, 0)  {$\Del(e)$};
      \node (fe)  at (4, -0.5)  {$\Flush(e)$};
      \node (df)  at (6, 0)  {$\Del(f)$};
      \node (ff)  at (6, -0.5)  {$\Flush(f)$};
    \end{scope}
		
    \path[->] (da) edge [out=225,in=135,dashed] node [left=0.1cm] {po} (db);
    \path[->] (fa) edge [out=225,in=135] node [left=0.1cm] {se} (fb);
    \path[->] (fb) edge [out=-30,in=225,looseness=1.0] node [below right=0.07cm] {se} (ff);
    \path[->] (dc) edge [out=225,in=135,dashed] node [left=0.1cm] {po} (dd);
    \path[->] (fc) edge [out=225,in=135] node [left=0.1cm] {se} (fd);
    \path[->] (fa) edge [out=37,in=142] node [above=0.1cm] {ue} (fe);
    \path[->] (fd) edge [out=30,in=-120] node [above left=0.07cm] {se} (fe);
    \path[->] (fc) edge [out=37,in=142] node [above=0.1cm] {ue} (ff);
  \end{tikzpicture}}
  \caption{IRIW+dps}
  \label{fig:some}
\end{figure}


==> implementation-back.tex <==
% vi: filetype=tex spell spelllang=en_gb:
\section{Implementation\label{implementation}}

To achieve a high degree of automation, we implemented the instrumentation
technique described above.  Our tool reads a concurrent C program, and
generates a new concurrent C program augmented with buffers and queues,
which is then passed to an SC verification tool.  We added two memory fences
({\tt fence} and {\tt lwfence}) as new keywords to support x86's {\tt
mfence} and Power's {\tt sync} and {\tt lwsync} with the semantics presented
in~\mysec\ref{context}.  The instrumentation tool also allows us to
visualise the cycles that the program exhibits, and optionally to restrict
the pairs to instrument in order to improve the performance of the program
analysers.

We provide an overview of our setup in~\myfig\ref{fig:tool}. We first
translate the C source code into a \emph{goto-program} (CProver's internal
representation), then feed it to \prog{goto-instrument} (a tool for
automating transformations of goto-programs).  We have extended
\prog{goto-instrument} with the instrumentation described in
\mysec\ref{instrumentation}: given a memory model (x86/TSO, PSO, RMO and
Power are available for now), \prog{goto-instrument} adds the
instructions necessary to instrument the delay pairs, taking fences into
account (and removing them).

\begin{figure}[!t]
\scalebox{0.7}{
\begin{tikzpicture}

  \tikzstyle{state} = [draw, very thick, fill=white, rectangle,
     minimum height=3em, minimum width=7em, node distance=13em,
     rounded corners]
  \tikzstyle{stateOption} = [node distance=1em]
  \tikzstyle{stateEdgePortion} = [black,thick];
  \tikzstyle{stateEdge} = [stateEdgePortion,->];
  \tikzstyle{edgeLabel} = [pos=0.5, above=0.2em, text centered];

  \node[state, name=cfile] {C file};
  \node[state, name=gotocc, right of=cfile] {goto-cc};

  \node [below of=gotocc, name=4] {+ \emph{fence}};
  \node [below of=4, name=5, stateOption] {+ \emph{lwfence}};

  \node[state, name=gotoinst, right of=gotocc] {goto-instrument};

  \node [below of=gotoinst, name=1] {+ memory model};
  \node [below of=1, name=2, stateOption] {+ 1 pair per cycle/all pairs};
  \node [below of=2, name=3, stateOption] {+ pairs to instrument};
  \node [below of=3, name=4, stateOption] {+ detect dependencies};

  \node[state, name=mc, right of=gotoinst] {SC verification tool};

  \node[state, name=cdump, right of=gotoinst, left of=mc, above of=mc, node distance=9em] {goto-instrument --dump-c};
  \node[state, name=graph, above of=gotoinst, node distance=9em] {graph};

  \draw (cfile) edge [stateEdge] (gotocc) {};
  \draw (gotocc) edge [stateEdge] node [edgeLabel] {goto-pg.} (gotoinst) {};
  \draw (gotoinst) edge [stateEdge] node [edgeLabel,left=0.5em] {goto-pg.} (cdump) {};
  \draw (gotoinst) edge [stateEdge, dashed] node [edgeLabel] {goto-pg.}(mc) {};
  \draw (cdump) edge [stateEdge] node [edgeLabel, right=1.5em, name=6]  {C code augmented w.r.t.} (mc) {}; 
  \node [text centered, below of=6, node distance=1em] {instrumentation of \mysec\ref{instrumentation}};
  \draw (gotoinst) edge [stateEdge] (graph) {};  

\end{tikzpicture}
}
\caption{Overview of our tool chain. 
%{\small *We added \emph{fence} and \emph{lwfence} to goto-cc. 
\label{fig:tool}}
\vspace*{-3mm}
\end{figure}
%  \node [below of=mc, name=5] {+ SATABS};
%  \node [below of=5, name=6, stateOption] {+ C-IMPACT};
%  \node [below of=6, name=7, stateOption] {+ ESBMC};
%  \node [below of=7, name=8, stateOption] {+ THREADER};

To perform the instrumentation, \prog{goto-instrument} first produces a
graph of events from the program.  This graph over-approximates the event
structures, in that it ignores all the values the variables may hold.  This
can lead to some spurious cycles (cf.~\mysec\ref{experiments}), but this
does not impair the soundness of our method.

The tool then computes the cycles that contain delay pairs for the selected
memory model, and instruments reads and writes using a buffer of size $2$
for each variable.  It also inserts assertions after the buffer
instrumentations to ensure that the buffer bound is never exceeded.
The instrumenter implements a very simple analysis to detect the
dependencies between the variables of a given thread to compute the $\dep$
relation of~\mysec\ref{context}.  This allows us to eliminate thin air
cycles.  The alias analysis used for this step is non-relational and thus
sound w.r.t.~weak memory~\cite{DBLP:conf/aplas/AlglaveKLNT11}.

In order to quantify the benefit of the optimisation proposed in
\mysec\ref{sec:reduced}, we offer several different instrumentation
strategies: \prog{goto-instrument} can instrument \emph{all} the delay pairs
(following \mythm\ref{thm:equiv}), or only one pair per cycle (following
\mythm\ref{thm:optim}).  As we discuss in \mysec\ref{experiments}, this
choice can have a drastic impact on the time required by the program
analyser.

The instrumented goto-program is directly amenable to Model Checking using
analysers that can read this format (\eg CImpact or SatAbs). 
Alternatively, we can convert it back into C code with the option {\tt
--dump-c}, and hand it to any Model Checker that can read C source (\eg
CheckFence, ESBMC, Poirot, Threader).  To be able to experiment with
Blender, we also wrote a converter to generate a format readable by Blender.


